Spiking Transformer Hardware Accelerators in 3D Integration

Spiking neural networks (SNNs) are powerful models of spatiotemporal computation and are well suited for deployment on resource-constrained edge devices and neuromorphic hardware due to their low power consumption. Leveraging attention mechanisms similar to those found in their artificial neural network counterparts, recently emerged spiking transformers have showcased promising performance and efficiency by capitalizing on the binary nature of spiking operations. Recognizing the current lack of dedicated hardware support for spiking transformers, this paper presents the first work on 3D spiking transformer hardware architecture and design methodology. We present an architecture and physical design co-optimization approach tailored specifically for spiking transformers. Through memory-on-logic and logic-on-logic stacking enabled by 3D integration, we demonstrate significant energy and delay improvements compared to conventional 2D CMOS integration.

==> features.tex <==
\begin{table*}[!tbp]
    \centering
    \caption{Comparison of Neuromorphic Hardware}
    \begin{tabular}{c l c c c}
    \toprule
       Group & Property                     &  GPBO     & LLMBO     & Proposed \ourmethod    \\
   \midrule
       Domain knowledge & Circuit topology            & No    & Yes    & Yes        \\ 
        & Design principle         & No    & Yes    & Yes        \\ 
                 & Region of operation      & No    & Yes    & Yes        \\   
        & Sub-circuit tuning               & No    & Yes    & Yes        \\
        & Validity of design choice               & Low    & High    & High        \\
    \midrule
        General ability & \makecell[l]{Scalability to large dataset}       & High    & Low    & High        \\
        & Computation efficiency               & High    & Low    & High        \\
                & Exploration (?)               & High & Low & High\\
                & Exploitation (?)               & Low & High & High\\
                & Multi-objective optimization & Low    & High & High \\
\bottomrule
    \end{tabular}
    \label{tab:bo-properties}
\end{table*}

